Truthful Mechanisms for Combinatorial AC Electric Power Allocation

Traditional studies of combinatorial auctions often only consider linear constraints (by which the demands for certain goods are limited by the corresponding supplies). The rise of smart grid presents a new class of auctions, characterized by quadratic constraints. Yu and Chau [AAMAS 13'] introduced the complex-demand knapsack problem, in which the demands are complex-valued and the capacity of supplies is described by the magnitude of total complex-valued demand. This naturally captures the power constraints in AC electric systems. In this paper, we provide a more complete study and generalize the problem to the multi-minded version, beyond the previously known 1/2-approximation algorithm for only a subclass of the problem. More precisely, we give a truthful PTAS for the case phi in [0,pi/2-delta], and a truthful FPTAS, which fully optimizes the objective function but violates the capacity constraint by at most (1+epsilon), for the case phi in (pi/2,pi-delta], where phi is the maximum angle between any two complex-valued demands and epsilon,delta>0 are arbitrarily small constants.

==> bi-fptas.tex <==
\section{Bi-criteria FPTAS for \textsc{CKP$[0,\pi\mbox{-}\varepsilon]$}} \label{sec:bfptas} 

In the previous section, we have restricted our attention to the setting where all demands lie in the positive quadrant in the complex plane (i.e., \textsc{CKP$[0,\frac{\pi}{2}]$}). In this section, we extend our study to the second quadrant (\textsc{CKP$[0,\pi\mbox{-}\varepsilon]$}) for any $\varepsilon > 0$, that is, we assume ${\rm arg}(d_k) \le \pi-\varepsilon$ for all $k \in \cN$. We note that the next section shows that \textsc{CKP$[0, \pi]$} is inapproximable and 
there is no $(\alpha, 1)$-approximation for \textsc{CKP$[0,\pi \mbox{-} \varepsilon]$}. Therefore, we can at best obtain a bi-criteria approximation, and furthermore the running time should depend on the maximum angle $\phi\triangleq\max_k{\rm arg}(d_k)$.

For convenience, we let $\theta = \max\{\phi - \frac{\pi}{2},0\}$
%, such that ${\rm arg}(d_k) \le \theta + \frac{\pi}{2}$ for all $k \in \cN$
 (see Fig.~\ref{f4} for an illustration).
\begin{figure}[!htb]
	\begin{center}
		\includegraphics{fig/fig4.pdf}
	\end{center}
\caption{All demands lie in the shaded area. We measure $\theta = \phi - \frac{\pi}{2}$ from the imaginary axis.}
	\label{f4}
\end{figure}
 

We present a  $(1,1+\epsilon)$-approximation  for \textsc{CKP$[0,\pi\mbox{-}\varepsilon]$} in Algorithm {\sc CKP-biFPTAS} that is polynomial in both $\frac{1}{\epsilon}$ and $n$ (i.e., FPTAS). We assume that $\tan \theta$ is bounded polynomial $P(n)\ge 1$ in $n$; as we will see in the next section, without this assumption, a bi-criteria FPTAS is unlikely to exist. 

Let $\cN_+\triangleq \{k \in \cN \mid d_k^{\rm R} \ge 0\}$ and $\cN_-\triangleq\{k \in \cN \mid d_k^{\rm R} < 0\}$ be the subsets of users with demands in the first and second quadrants respectively. Consider any  solution $S$ to \textsc{CKP$[0,\pi\mbox{-}\varepsilon]$} and define $S_+ \triangleq \{ k \mid d_k^{\rm R} \ge 0, k \in S \}$ and $S_- \triangleq \{ k \mid   d_k^{\rm R} < 0, k \in S \}$ as the subsets of users with demands having non-negative and negative real components respectively. 

The basic idea of Algorithm {\sc CKP-biFPTAS} is to enumerate the guessed total projections on real and imaginary axes for $S_+^\ast$ and $S_-^\ast$ respectively. 
We can use $\tan \theta$ to upper bound the total projections for any feasible subset $S$ as follows:
\begin{align}
 \sum_{k \in S} d_k^{\rm I} \le C, \quad
 \sum_{k \in S_- } - d_k^{\rm R}   \le  C \tan \theta, \quad 
 \sum_{k \in S_+}  d_k^{\rm R}   &\le C(1+ \tan \theta). \label{eq:ubounds}
\end{align}
We then solve two separate {\sc 2DKP} problems (one for each quadrant) to find subsets of demands that satisfy the individual guessed total projections. But since {\sc 2DKP} is generally NP-hard, we need to round-up the demands to get a problem that can be solved efficiently by dynamic programming. We show that the violation of the optimal solution to the rounded problem w.r.t. to the original problem is small in $\epsilon$. 

Next, we describe the rounding in detail. First, we define\footnote{For a more efficient procedure, we may replace $P(n)$ by $\max\{\tan \theta,1\}$; however, choosing $L$ to depend only on $P(n)$, and thus independent of the demands, will be needed for the truthful mechanism in Sec. \ref{sec:tbp}} $L \triangleq \frac{\epsilon C}{n (P(n)+1)}$, such that the new rounded-up demands $\hat{d_k}$ are defined by:
\begin{equation}
\hat d_k =
\hat d_k^{\rm R} + {\bf i} \hat d_k^{\rm I} \triangleq 
\left\{\begin{array}{ll}
\left\lceil \frac{d_k^{\rm R}}{L} \right\rceil \cdot L + {\bf i} \left\lceil \frac{d_k^{\rm I}}{L} \right\rceil \cdot L, &\text{ if }d^{\rm R}_k\ge 0,\\[3mm]
\left\lfloor \frac{d_k^{\rm R}}{L} \right\rfloor \cdot L + {\bf i} \left\lceil \frac{d_k^{\rm I}}{L} \right\rceil \cdot L, & \text{ otherwise. } 
\end{array}\right.
\label{eq:truc}
\end{equation}
Let $\xi_+$ (and $\xi_-$), $\zeta_+$ (and $\zeta_-$) be respectively the guessed real and imaginary absolute total projections of the rounded demands in $S^\ast_+$ (and $S_-^\ast$).
%\begin{equation}
%\xi_+ \triangleq \{ d_k^{\rm R} \mid  k \in S_+ \}, \  \zeta_+ \triangleq \{ d_k^{\rm I} \mid  k \in S_+ \}, \ \xi_- \triangleq \{ - d_k^{\rm R} \mid  k \in S_- \}, \  \zeta_- \triangleq \{ %d_k^{\rm I} \mid  k \in S_- \}
%\end{equation}
Then the possible values of $\xi_+, \xi_-, \zeta_+$ and $\zeta_-$ are integer mutiples of $L$:
\begin{align}
 \xi_+ \in {\cal A}_+ & \triangleq \left\{0, L, 2L,\ldots,\left\lceil \frac{C (1 + P(n) )}{L} \right\rceil \cdot L\right\},\ 
\xi_- \in {\cal A}_- \triangleq \left\{0,L, 2L,\ldots, \left\lceil \frac{C \cdot P(n) }{L} \right\rceil\cdot L \right\}, \nonumber \\
\zeta_+,\zeta_-  \in {\cal B} & \triangleq \left\{0, L, 2L,\ldots,\left\lceil \frac{C}{L} \right\rceil\cdot L.\right\}
\label{eq:grid}
\end{align}
%Note that a feasible guess of total projections should satisfy constraint Eqn.~\raf{C1} for \textsc{CKP}, and thus:
%\begin{equation}\label{eq:sat}
%(\xi_+ - \xi_-)^2 + (\zeta_+ + \zeta_-)^2 \le (1+2\epsilon)^2C^2;
%\end{equation}
%see Lemma~\ref{lem-trunc} below. 
%Step \ref{alg:tight} forces the corresponding selected demands to be tight; otherwise, constraint Eqn.~\raf{C1} could be violated largely. Now, for each guess, we consider solving two {\sc 2DKP} instances separately. The first one with capacities $\xi_+$, $\zeta_+$ and positive demands $\hat d_k, k \in \cN_+$, and the second with $\xi_-,\zeta_-$ and demands in $\cN_-$. 


The next step is to solve the rounded instance exactly. Assume an arbitrary order on $\cN = \{ 1, ..., n\}$. We use recursion to define a 3D table, with each entry ${U}(k,c_1, c_2)$ as the maximum utility obtained from a subset of users $\{1,2,\dots,k\} \subseteq \cN$ with demands $\{\hat{d_1},\hat{d_2},...,\hat{d_k}\}$ that can fit exactly (i.e., satisfies the capacity constraint as an equation) within capacity $c_1$ on the real axis and $c_2$ on the imaginary axis. 
\iffalse
The cells are defined according to the following rules:
\begin{align}
{U}(1,C_1, C_2) &\triangleq  \left\{ \begin{array}{l l}
u_k & \quad \text{if $\hat{d_k^{\rm R}} = C_1$ and $\hat d_k^{\rm I}  = C_2$}\\
-\infty &\quad \text{otherwise} \end{array}\right.\label{eq:dyn-rule1}\\
{U}(i+1,C_1, C_2) &\triangleq \max  \left\{ \begin{array}{l}
u_{i+1} + {U}(i, C_1 - \hat d_k^{\rm R}, C_2 - \hat d_k^{\rm I}),\\
{U}(i,C_1,C_2)
 \end{array}\right.
 \label{eq:dyn-rule2}
\end{align}
\fi
We denote by {\sc 2DKP-Exact}$[\cdot]$ the algorithm for solving {\sc 2DKP} by dynamic programming.


\begin{algorithm}[!htb]
\caption{{\sc CKP-biFPTAS} $( \{u_k,d_k\}_{k \in \cN}, C,\epsilon) $}\label{CKP-biFPTAS}
\begin{algorithmic}[1]
\Require Users' utilities and demands $\{u_k,d_k\}_{k\in \cN}$; capacity $C$; accuracy parameter $\epsilon$
\Ensure $(1,1+3\epsilon)$-solution $\hat{S}$ to \textsc{CKP$[0,\pi\mbox{-}\varepsilon]$}
\State $\hat{S} \leftarrow \varnothing$.
\ForAll {$d_k$ and $k \in \cN$}
\State Set $\hat d_k \leftarrow \hat d_k^{\rm R} + {\bf i} \hat d_k^{\rm I} $ as defined by \raf{eq:truc}
\EndFor
\ForAll {$\xi_+ \in {\cal A}_+, \xi_- \in {\cal A}_-, \zeta_+, \zeta_- \in {\cal B}$}
\If {$(\xi_+ - \xi_-)^2 + (\zeta_+ + \zeta_-)^2 \le (1+2\epsilon)^2C^2$}\label{cond1}
\State $\qquad F_+ \leftarrow \text{\sc 2DKP-Exact}(\{u_k,\hat d_k/L\}_{k\in\cN_+}, \xi_+/L,\zeta_+/L)$
 \State $\qquad F_- \leftarrow \text{\sc 2DKP-Exact}(\{u_k,-\hat d_k/L\}_{k\in \cN_-}, \xi_-/L,\zeta_-/L)$ 
%\If{$F_+, F_- \neq \varnothing$} \label{alg:tight}
\If{$u(F_+ \cup F_-) > u (\hat{S})$}
\State $\hat{S} \leftarrow  \{F_+ \cup F_-\}$
\EndIf 
%\EndIf 
\EndIf
\EndFor
\State \Return $\hat{S}$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!htb]
\caption{{\sc 2DKP-Exact} $( \{u_k,\hat d_k\}_{k \in \cN'}, C_1,C_2) $}
\begin{algorithmic}[1] 
\Require Users' utilities and integer demands $\{u_k,\hat d_k\}_{k\in \cN'}$; integer capacities $C_1,C_2$
\Ensure A utility-maximizing subset of satisfiable users $\subseteq \cN'$ subject to capacity constraints defined by $C_1,C_2$
\State Create a 3D table of size $|\cN'| \times (C_1+1) \times (C_2+1)$, with each entry ${U}(k,c_1, c_2)$ according to: 
\begin{align}
{U}(1,c_1, c_2) &\triangleq  \left\{ \begin{array}{l l}
u_1 & \quad \text{if $\hat d_1^{\rm R} = c_1$ and $\hat d_1^{\rm I}  = c_2$}\\
-\infty &\quad \text{otherwise} \end{array}\right.\label{eq:dyn-rule1}\\
U(k, 0, 0) &\triangleq 0 ~~\text{ and }~~U(k, c_1', c_2') \triangleq -\infty\text{ for all }c_1'<0 \text{ or } c_2'<0\\
{U}(k,c_1, c_2) &\triangleq \max  \left\{ 
u_{k} + {U}(k-1, c_1 - \hat d_k^{\rm R}, c_2 - \hat d_k^{\rm I}),
{U}(k-1,c_1,c_2) \right\}
 \label{eq:dyn-rule2}
\end{align}
\State Create a 3D table of size $|\cN'| \times C_1 \times C_2$, with each each entry ${\cI}(k,c_1, c_2)$ according to: 
\begin{align}
\cI(1,c_1, c_2) &\triangleq \left\{\begin{array}{l l}
\{1 \}& \ \text{if $U(1,c_1,c_2) = u_1$}\\
\varnothing & \ \text{otherwise} 
\end{array}\right.\\
{\cI}(k,c_1, c_2) &\triangleq  \left\{ \begin{array}{ll}
{\cI}(k-1,c_1, c_2) &\  \text{if ${U}(k,c_1, c_2) = {U}(k-1, c_1, c_2)$} \\
{\cI}(k-1,c_1- \hat d_k^{\rm R}, c_2- \hat d_k^{\rm I}) \cup \{ k \} &\  \text{if ${U}(k,c_1, c_2) = u_{k} + {U}(k-1, c_1 - \hat d_k^{\rm R}$}, c_2 - \hat d_k^{\rm I}) \\
\end{array}\right.
 \label{eq:dyn-rule3}
\end{align}
\State \Return $\displaystyle {\cI}(n,C_1,C_2)$.
\end{algorithmic}
\end{algorithm}


\begin{theorem}\label{thm:bptas}
Algorithm {\sc CKP-biFPTAS} is $(1,1+3\epsilon)$-approximation for \textsc{CKP$[0,\pi\mbox{-}\varepsilon]$} and its running time is polynomial in both $n$ and $\frac{1}{\epsilon}$.
\end{theorem}
\begin{proof}
First, the running time is proportional to the number of guesses, upper bounded by $O(\frac{1}{\epsilon^4} n^{4} P^6(n))$. For each guess, {\sc 2DKP-Exact} constructs a table of size at most $O(\frac{1}{\epsilon^2} n^3 P^4(n))$. Since we assumed $P(n)$ is polynomial in $n$, the total running time is polynomial in $n$ and $\frac{1}{\epsilon}$.

To show the approximation ratio of 1, we note {\sc CKP-biFPTAS} enumerates over all possible rounded projections subject to the capacity constraint in {\sc CKP} and that {\sc 2DKP-Exact} returns the exact optimal solution for each rounded problem. In particular, by Lemma \ref{lem-trunc} one of the choices would be rounded projection for the optimum solution $S^\ast$.   
It remains to show that the violation of the returned solution is small in $\epsilon$. This is given in Lemma~\ref{lem-trunc2} below, which shows that the solution $\hat S$ to the rounded problem violates the capacity constraint by only a factor at most $(1+3\epsilon)$. 
\end{proof}

%In fact, $\epsilon$ is inversely proportional to $\theta$. The larger $\theta$ the smaller $\epsilon$ is required for maintaining the precision. This can be observed from Eqn.~\raf{lem1-p2}.

For any set $S\subseteq\cN$, let us write $D_+(S)\triangleq\sum_{k\in S_+}d_k^{\rm R}$, $D_-(S)\triangleq\sum_{k\in S_-}-d_k^{\rm R}$, $D_I(S)\triangleq\sum_{k\in S}d_k^{\rm I}$, $\hat D_+(S)\triangleq\sum_{k\in S_+} \hat d_k^{\rm R}$, $\hat D_-(S)\triangleq\sum_{k\in S_-} -\hat d_k^{\rm R}$, and $\hat D_I(S)\triangleq\sum_{k\in S}\hat d_k^{\rm I}$. Then by \raf{eq:truc} and the fact that $x \le t \lceil \frac{x}{t} \rceil  \le x + t$ for any $x,t$ such that $t>0$, we have 
\begin{eqnarray}\label{eq:bds}
&\max\{\hat D_+(S)-L|S|,0\}\le D_+(S)\le \hat D_+(S),~~~\max\{\hat D_-(S)-L|S|,0\}\le D_-(S)\le \hat D_-(S), \nonumber \\ & \max\{\hat D_I(S)-L|S|,0\}\le D_I(S)\le\hat D_I(S).
\end{eqnarray}

\begin{lemma}
For any optimal solution $S^*$ to \textsc{CKP$[0,\pi\mbox{-}\varepsilon]$}, $L\triangleq \frac{\epsilon C}{nP(n)}$ and $\epsilon> 0$, we have
\begin{equation}
 \left( \sum_{k \in S^*} \hat d_k^{\rm R} \right)^2 +  \left(\sum_{k \in S^*} \hat   d_k^{\rm I} \right)^2  \le C^2 ( 1 + 2\epsilon)^2 .
 \label{eq:lem}
\end{equation}
 \label{lem-trunc}
\end{lemma}
\begin{proof}
%First, we note that any optimal solution $S^*$ satisfies constraint Eqn.~\raf{C1}:
%\begin{equation}
%\left(\sum_{k\in S^*} d_k^{\rm R} \right)^2 + \left( \sum_{k \in S^* } d_k^{\rm I}\right)^2 \le C^2
%\label{eq:C1}
%\end{equation}


Using~\raf{eq:bds},
\begin{align}
\left( \sum_{k \in S^*} \hat d_k^{\rm R} \right)^2 +  \left(\sum_{k \in S^*} \hat d_k^{\rm I} \right)^2 &=\left(\hat D_+(S^*)- \hat D_-(S^*)\right)^2 +  \hat D_I^2(S^*)\nonumber\\
&=\hat D_+^2(S^*)+\hat D_-^2(S^*)-2\hat D_+(S^*)\hat D_-(S^*)+\hat D_I^2(S^*)\nonumber\\ 
&\le (D_+(S^*)+nL)^2+(D_-(S^*)+nL)^2-2D_+(S^*) D_-(S^*)+(D_I(S^*)+nL)^2\nonumber\\
&=(D_+(S^*)-D_-(S^*))^2+D_I^2(S^*)+2nL (D_+(S^*)+D_-(S^*)+D_I(S^*))+3n^2L^2\nonumber\\
&= \left(\sum_{k\in S^*} d_k^{\rm R} \right)^2 + \left(\sum_{k\in S^*} d_k^{\rm I}  \right)^2 +2nL\left(\sum_{k\in S^*}|d_k^{\rm R}|+\sum_{k\in S^*}d_k^{\rm I}\right)+3n^2L^2\nonumber\\
&\le C^2 + 4nL (P(n)+1) C + 3n^2L^2 = C^2 + 4 \epsilon C^2 + 3\epsilon^2 C^2/(1+P(n))^2\nonumber \\ &\le C^2 (1+4\epsilon + \epsilon^2)\le C^2(1+2\epsilon)^2\label{lem1-p2}.
\end{align}
\end{proof}

\begin{lemma}\label{lem-trunc2}
Let $\hat S$ be the solution returned by {\sc CKP-biFPTAS}. Then $|\sum_{k\in\hat S}d_k|\le(1+3\epsilon) C$. 
\end{lemma}
\begin{proof}
As in~\raf{lem1-p2},
\begin{align}\label{eq:ee1}
\left( \sum_{k \in \hat S} d_k^{\rm R} \right)^2 +  \left(\sum_{k \in \hat S} d_k^{\rm I} \right)^2 &=\left(D_+(\hat S)- D_-(\hat S)\right)^2 +  D_I^2(\hat S)\nonumber\\
&=D_+^2(\hat S)+D_-^2(\hat S)-2D_+(\hat S)D_-(\hat S)+D_I^2(\hat S).
\end{align} 
If both $\hat D_+(\hat S)$ and $\hat D_-(\hat S)$  are less than $nL$, then the R.H.S. of \raf{eq:ee1} can be bounded by 
\begin{align}\label{eq:ee2}
&\hat D_+^2(\hat S)+\hat D_-^2(\hat S)+\hat D_I^2(\hat S)
\le\hat D_+^2(\hat S)+\hat D_-^2(\hat S)-2\hat D_+(\hat S)\hat D_-(\hat S)+2n^2L^2+\hat D_I^2(\hat S)\nonumber\\
&=(\hat D_+(\hat S)-\hat D_-(\hat S))^2+\hat D_I^2(\hat S)+2n^2L^2.
\end{align}
Otherwise, we bound the R.H.S. of \raf{eq:ee1} by
\begin{align}\label{eq:ee3}
&\hat D_+^2(\hat S)+\hat D_-^2(\hat S)-2(\hat D_+(\hat S)-nL)(\hat D_-(\hat S)-nL)+\hat D_I^2(\hat S)\nonumber\\
&=(\hat D_+(\hat S)-\hat D_-(\hat S))^2+\hat D_I^2(\hat S)+2nL(\hat D_+(\hat S)+\hat D_-(\hat S))-2n^2L^2.
\end{align}
Since $\hat S=F_+\cup F_-$ is obtained from feasible solutions $F_+$ and $F_-$ to $\text{\sc 2DKP-Exact}(\{u_k,\hat d_k/L\}_{k\in\cN_+}, \xi_+/L,\zeta_+/L)$
 and $\text{\sc 2DKP-Exact}(\{u_k,-\hat d_k/L\}_{k\in \cN_-}, \xi_-/L,\zeta_-/L)$, respectively, and  $\xi_+ , \xi_-,\zeta_+, \zeta_-$ satisfy the condition in Step~\ref{cond1}, it follows from \raf{eq:ee1}-\raf{eq:ee3} that
\begin{align*}
\left( \sum_{k \in \hat S} d_k^{\rm R} \right)^2 +  \left(\sum_{k \in \hat S} d_k^{\rm I} \right)^2 &\le \left( \sum_{k \in \hat S} \hat d_k^{\rm R}\right)^2 +  \left(\sum_{k \in \hat S}\hat d_k^{\rm I} \right)^2+2nL\sum_{k \in \hat S_-} |\hat d_k^{\rm R}|+2n^2L^2\nonumber\\
&=(\xi_+ - \xi_-)^2 + (\zeta_+ + \zeta_-)^2 + 2nL\xi_-+2n^2L^2\nonumber\\
&\le \left((1+2\epsilon)^2C^2 +2n\frac{\epsilon}{n(P(n)+1)} C^2 + 2n^2\frac{\epsilon^2}{n^2(P(n)+1)^2}\right)C^2\\
&\le \left((1+2\epsilon)^2 +\epsilon + \frac{\epsilon^2}{2}\right)C^2\le (1+3\epsilon)^2C^2.
\end{align*}
\end{proof}

\iffalse
\begin{corollary}
For any $(\alpha, \beta)$-approximation algorithm of \textsc{CKP$[0,\pi\mbox{-}\varepsilon]$} using truncated demands $\hat d_k$, we have $(\alpha, \beta (1+\epsilon))$-approximation for original demands $d_k$.
\label{cor} 
\end{corollary}
This follows immediately from Lemma~\ref{lem-trunc}. The approximation ratio $\alpha$ remains the same since any optimal $S^*$ is also feasible in the new instance within a violation of $(1+\epsilon)$.
\fi

